Modelling astrophysical fluids with particles

Computational fluid dynamics is a crucial tool to theoretically explore the cosmos. In the last decade, we have seen a substantial methodological diversification with a number of cross-fertilizations between originally different methods. Here we focus on recent developments related to the Smoothed Particle Hydrodynamics (SPH) method. We briefly summarize recent technical improvements in the SPH-approach itself, including smoothing kernels, gradient calculations and dissipation steering. These elements have been implemented in the Newtonian high-accuracy SPH code MAGMA2 and we demonstrate its performance in a number of challenging benchmark tests. Taking it one step further, we have used these new ingredients also in the first particle-based, general-relativistic fluid dynamics code that solves the full set of Einstein equations, SPHINCS_BSSN. We present the basic ideas and equations and demonstrate the code performance at examples of relativistic neutron stars that are evolved self-consistently together with the spacetime.

==> own_latex_commands_i.tex <==
% own commands
\newcommand{\nifs}{\ensuremath{^{56}\mathrm{Ni}}}
\newcommand{\Nifs}{\ensuremath{^{56}\mathrm{Ni}} $\;$}
\def\paren#1{\left( #1 \right)}
\def\Mesz{M\'esz\'aros~}
\def\Pacz{Paczy\'nski~}
\def\Kluz{Klu\'zniak~}
\def\p{\partial}
\def\msun{M$_{\odot}$}
\def\Msun{M$_{\odot}$ }
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bi{\begin{itemize}}
\def\i{\item}
\def\ei{\end{itemize}}
\def\ben{\begin{enumerate}}
\def\een{\end{enumerate}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\bt{\begin{tabbing}}
\def\et{\end{tabbing}}
\def\gcc{gcm$^{-3}$}
\def\Gcc{gcm$^{-3} \;$}
\def\ccm{cm$^3$}
\def\edo{\end{document}}
\def\red{\textcolor{red}}
\def\blue{\textcolor{blue}}
\def\green{\textcolor{green}}
\def\ye{$Y_e$}
\def\Ye{$Y_e$ }
\def\rs{$R_{\rm S}$}
\def\Rs{$R_{\rm S}$ }
\def\noin{\noindent}
\def\QIone{\mathcal{Q}_{\; \; 1}}
\def\QItwo{\mathcal{Q}_{\; \; 2}}
\def\QIthree{\mathcal{Q}_{\; \; 3}}
\def\QIfour{\mathcal{Q}_{\; \; 4}}
\newcommand{\ud}{\mathrm{d}}
\newcommand{\sn}{\ensuremath{\mathrm{sn}}}
\newcommand{\cn}{\ensuremath{\mathrm{cn}}}
\newcommand{\dn}{\ensuremath{\mathrm{dn}}}
\newcommand{\sech}{\ensuremath{\mathrm{sech}}}
\newcommand{\nd}{\noindent}
\newcommand{\enth}{\mathcal{E}}
\newcommand{\carb}{$^{12}$C}
\newcommand{\Carb}{$^{12}$C $\;$}
\newcommand{\ox}{$^{16}$O}
\newcommand{\Ox}{$^{16}$O $\;$}
\newcommand{\tlg}{\tilde{\gamma}}
\newcommand{\tlG}{\tilde{\Gamma}}
\newcommand{\emfp}{e^{-4\phi}}
\newcommand{\tlA}{\tilde{A}}
\newcommand{\tlR}{\tilde{R}}
\newcommand{\xt}{\tilde{x}}
\newcommand{\dt}[1]{\partial_t #1}
\newcommand{\pdu}[3]{\partial_{#3} #1^{#2}}
\newcommand{\pdl}[3]{\partial_{#3} #1_{#2}}
\newcommand{\pdpdu}[4]{\partial_{#3}\partial_{#4} #1^{#2}}
\newcommand{\pdpdl}[4]{\partial_{#3}\partial_{#4} #1_{#2}}
\newcommand{\upwindu}[3]{\beta^{#3}\bar{\partial}_{#3} #1^{#2}}
\newcommand{\upwindl}[3]{\beta^{#3}\bar{\partial}_{#3} #1_{#2}}
%\newcommand{\comment}[1]{{\color{red}$\blacksquare$~\textsf{[#1]}}}
\newcommand{\tlGn}{\tilde{\Gamma}_{\mathrm{(n)}}}
\newcommand{\tlGmixed}[2]{\tlG_{#1}^{\;\;\;#2}}



% Oleg's special
\def\peak{\rm peak}
\def\ji{\varphi}
\def\rin{\mathcal{I}}
\def\x{{\bf x}}
\def\s{{\bf s}}
\def\k{{\bf k}}
\def\n{{\bf n}}
\def\f{{\bf f}}
\def\pd{\partial}
\def\fa{f_{\alpha}(\x,\p,t)}
\def\kabs{\kappa^{\rm abs}_\nu}
\def\ksca{\kappa^{\rm sca}_\nu}
\def\Flux{{\bf F}_\nu}
\def\Frad{{\bf F}_{\rm rad}}
\def\Pressure{{\mathsf P}_\nu}
\def\kB{k_B}
\def\tauph{\tau_{\it ph}}
\def\taumu{\tau_\mu}
\def\MSun{M_{\astrosun}}


% Journals
\newcommand{\apj}{Ap. J., }
\newcommand{\apjl}{Ap. J. Lett., }
\newcommand{\apjs}{Ap. J. Supp., }
\newcommand{\physrep}{Phys. Rep., }
\newcommand{\mnras}{Mon. not. RAS., }
\newcommand{\apss}{Astroph. \& Space Sci., }
\newcommand{\aap}{Astron. \& Astrophys., }
\newcommand{\prc}{Phys. Rev. C.,} 
\newcommand{\prd}{Phys. Rev. D.,} 
\newcommand{\nat}{Nature,}
\newcommand{\pasp}{Publications of the Astronomical Society of the Pacific,}

% SPH kernels
\def\M4{M$_4$}
\def\M6{M$_6$}
\def\lcm6{LCM$_6$}
\def\qcm6{QCM$_6$}
\def\whn{W$_{\rm H,n}$}
\def\wh3{W$_{\rm H,3}$}
\def\wh4{W$_{\rm H,4}$}
\def\wh5{W$_{\rm H,5}$}
\def\wh6{W$_{\rm H,6}$}
\def\wh7{W$_{\rm H,7}$}

% vector algebra
\def\divv{\nabla \cdot \vec{v}}
\def\vv{\vec{v}}
\def\dx{\Delta x}

% alternative vector symbole
\newcommand{\ve}[1]{\boldsymbol{#1}}

% turbulence
\def\ed{\dot{\epsilon}}
\def\vl{v_\lambda}
\def\vort{\vec{\mathcal{W}}}

% reduced quadrupole moment
\newcommand{\rqm}{{%
      \declareslashed{}{\text{-}}{0.04}{0}{I}\slashed{I}}}

% code names
\newcommand{\SpB}{\texttt{SPHINCS\_BSSN}\; }
\newcommand{\spB}{\texttt{SPHINCS\_BSSN}}
\newcommand{\Ma}{\texttt{MAGMA2}\;}
\newcommand{\ma}{\texttt{MAGMA2}}
\newcommand{\Lo}{\texttt{LORENE}\;}
\newcommand{\lo}{\texttt{LORENE}}
\newcommand{\comp}{\texttt{CompOSE}\;}
\newcommand{\binns}{\texttt{BinNS}\;}
\newcommand{\McL}{\texttt{McLachlan}\;}







